Dual-Source Latent Memory Weaving for Vision-Language-Action Models

Mainstream Vision-Language-Action (VLA) models predict actions primarily from the current observation under a Markovian assumption, thus struggling with long-horizon, temporally dependent tasks. Existing memory-augmented VLAs either expand the observation window or retrieve history from the memory bank as auxiliary policy-side context. However, they leave memory outside the native latent embedding space of VLA reasoning, preventing historical experience from being fluidly interleaved with multimodal reasoning and action formation. To this end, we introduce LaMem-VLA, a latent-memory-native framework that reconstructs historical experience into latent memory tokens and directly interweaves them with VLA reasoning. At its core, LaMem-VLA introduces four coordinated components: (i) a curator that organizes historical experience into two complementary short-term and long-term memory vaults; (ii) a seeker that queries both vaults using the multimodal cognition to retrieve context-relevant evidence; (iii) a condenser that reconstructs the retrieved evidence into compact short-term and long-term latent memory tokens; and (iv) a weaver that injects these memory tokens with the current observation and instruction into one continuous embedding sequence. By representing, retrieving, and consuming historical experience entirely in the same continuous latent space, LaMem-VLA enables memory to directly participate in VLA reasoning and guide action generation under a bounded context. Extensive experiments on SimplerEnv and LIBERO demonstrate the superiority of our LaMem-VLA.

==> figs/attention_mech.tex <==
\begin{figure*}[t]
\centering\includegraphics[width=0.99\textwidth]{figs/memory.pdf}
    \vspace{-10pt}
    \caption{\small{\textbf{Visualization of the memory mechanism in the real-world Cover Block task} (\S\ref{supp:mech}). \ourmethod attends to historical frames revealing the original block location, providing temporal context for lifting the cup covering the now-occluded block.}}
    \label{fig:attention}
    \vspace{-7pt}
\end{figure*}

==> figs/case_general.tex <==
\begin{figure*}[t]
\centering\includegraphics[width=0.99\textwidth]{figs/realwork_gen.pdf}
    \vspace{-10pt}
    \caption{\small{\textbf{Qualitative results of \ourmethod on Real-World} (\S\ref{supp:qualitative}). From top to bottom, we illustrate three General Tasks: \textit{Stack cup}, \textit{Drawer}, and \textit{Pick fruit}.}}
    \label{fig:casegen}
    \vspace{-4pt}
\end{figure*}

==> figs/case_libero.tex <==
\begin{figure*}[t]
\centering\includegraphics[width=0.99\textwidth]{figs/case_libero.pdf}
    \vspace{-10pt}
    \caption{\small{\textbf{Qualitative results of \ourmethod on LIBERO tasks} (\S\ref{supp:qualitative}). Representative examples include tasks from Spatial, Object, Goal, Long-10, and Long-90 suites.}}
    \label{fig:caselibero}
    \vspace{-7pt}
\end{figure*}

==> figs/case_long.tex <==
\begin{figure*}[!t]
\centering\includegraphics[width=0.99\textwidth]{figs/realwork_long.pdf}
    \vspace{-10pt}
    \caption{\small{\textbf{Qualitative results of \ourmethod on long-horizon tasks} (\S\ref{supp:qualitative}). Representative examples include \textit{Cover block}, \textit{Press buttons}, and \textit{Fill drawer}.}}
    \label{fig:caselong}
    \vspace{-7pt}
\end{figure*}

==> tabs/ablation_latent_memory_tokens.tex <==



==> tabs/inference.tex <==
\begin{table*}[t]
\centering
\caption{
\small{\textbf{Inference efficiency comparison on an NVIDIA H20 GPU (\S\ref{supp:ablation}).}
Latency and peak GPU memory are averaged over 300 runs in bfloat16 with a batch size of 1 and an action chunk size of 16. Throughput denotes the number of actions generated per second.
}}
\label{tab:inference_efficiency}
\setlength{\tabcolsep}{10pt}
\resizebox{0.8\linewidth}{!}{
\setlength\tabcolsep{18pt}
\renewcommand\arraystretch{1.0}
\begin{tabular}{l|ccc}
\thickhline
\rowcolor{mygray}
\textbf{Model}
& \textbf{Latency (s)} $\downarrow$
& \textbf{Throughput (Hz)} $\uparrow$
& \textbf{Peak Memory (GB)} $\downarrow$ \\
\hline \hline
CogACT~\cite{li2024cogact} (Baseline) & 0.239s & 66.9Hz & 15.9GB \\
\ourmethod (Ours) & 0.315s & 50.8Hz & 17.8GB \\
\hline
\end{tabular}
}
\end{table*}



==> tabs/memory_merge.tex <==
% \begin{table}[t]
% \centering
% \caption{
% Ablation study of different memory updating strategies on the five LIBERO suites. All methods use the same fixed memory capacity.
% }
% \label{tab:memory_updating_strategy}
% \resizebox{\linewidth}{!}{
% \begin{tabular}{lccccc}
% \toprule
% \textbf{Updating Strategy}
% & \textbf{Spatial}
% & \textbf{Object}
% & \textbf{Goal}
% & \textbf{Long}
% & \textbf{LIBERO-90}
% \\
% \midrule
% FIFO
% & 97.8 & 98.2 & 92.8 & 90.6 & 93.6  \\

% Random Merge
% & 97.6 & 98.4 & 93.2 & 90.4 & -94.0 \\
% Adjacent Similarity Merge (\textbf{Ours})
% 98.8 &99.0 &97.2 &95.8 &97.0   \\
% \bottomrule
% \end{tabular}
% }
% \end{table}


% \begin{figure}[!t]
%     \centering
%     \includegraphics[width=0.7\textwidth]{figs/memory_strategy.pdf}
%     \vspace{-10pt}
%     \caption{\textbf{Ablation study of different memory vault updating strategies} on the five LIBERO suites~\cite{liu2023libero} (\S\ref{supp:ablation}). All methods use the same fixed memory capacity.
% }
%     \label{fig:strategy}
%     \vspace{-15pt}
% \end{figure}


\begin{figure}[t]
\vspace{-.5cm}
        \centering
		\includegraphics[width=1\linewidth]{figs/memory_strategy.pdf}
\captionsetup{font=small,width=1\linewidth}
 \vspace{-0.6cm}
 \caption{\small{\textbf{Ablation study of different memory vault updating strategies} on the five LIBERO suites~\cite{liu2023libero} (\S\ref{supp:ablation}). All methods use the same fixed memory capacity.
}}
    \label{fig:strategy}
\end{figure}

==> tabs/memory_size.tex <==
% \begin{table}[t]
% \centering
% \caption{
% Ablation on memory bank size. Results are average success rates (\%) on LIBERO-Long and Simple Env.
% }
% \label{tab:memory_bank_size}
% \setlength{\tabcolsep}{12pt}
% \begin{tabular}{c cc}
% \toprule
% \textbf{Memory Bank Size}
% & \textbf{LIBERO-Long}
% & \textbf{Simple Env.} \\
% \midrule
% 4  & 93.0 & 68.7 \\
% 8  & 94.4 & 70.8 \\
% 16 & 95.4 & 73.9 \\
% 32 & 95.8 & 71.9 \\
% 64 & 95.8 & 71.9 \\
% \bottomrule
% \end{tabular}
% \end{table}



% \begin{figure}[!t]
%     \centering
%     \includegraphics[width=0.5\textwidth]{figs/memory_bank_size.pdf}
%     \vspace{-10pt}
%     \caption{\textbf{Ablation study of memory bank size $L$} on SimplerEnv~\cite{li2025evaluating} and LIBERO-long~\cite{liu2023libero} (\S\ref{supp:ablation}).}
%     \label{fig:size}
%     \vspace{-15pt}
% \end{figure}

\begin{figure}[t]
\vspace{-.4cm}
        \centering
		\includegraphics[width=1\linewidth]{figs/memory_bank_size.pdf}
\captionsetup{font=small,width=1\linewidth}
 \vspace{-0.5cm}
  \caption{\small{\textbf{Ablation study of memory bank size $L$} on SimplerEnv~\cite{li2025evaluating} and LIBERO Long-90~\cite{liu2023libero} (\S\ref{supp:ablation}).}}
    \label{fig:size}
\end{figure}

==> tabs/real.tex <==
\begin{table*}[t]
\centering
\caption{
\textbf{Real-world evaluation results.}
We report the success rate (\%) on three generalization tasks and three long-horizon tasks.
}
\vspace{-5pt}
\label{tab:realworld_comparison}
\resizebox{\linewidth}{!}{
\setlength{\tabcolsep}{7pt}
\renewcommand{\arraystretch}{1.05}
\begin{tabular}{l|ccc|ccc}
\thickhline
\rowcolor{mygray}
\multirow{2}{*}{Method}
& \multicolumn{3}{c|}{Generalization Tasks}
& \multicolumn{3}{c}{Long-horizon Tasks} \\
\cline{2-7}
\rowcolor{mygray}
& Stack Cup
& Drawer
& Pick Fruit
& Cover Block
& Press Buttons
& Fill Drawer \\
\hline
\hline
OpenVLA~\citep{kim2024openvla}
& 38 & 42 & 24 & 10 & 14 & 14 \\

$\pi_0$~\citep{black2024pi_0}
& 62 & 68 & 66 & 26 & 36 & 36 \\

CogACT~\citep{li2024cogact}
& 78 & 66 & 62 & 38 & 48 & 52 \\

MemoryVLA~\citep{shi2025memoryvla}
& 78 & 72 & 66 & 34 & 54 & 50 \\
\hline
\textbf{LaMemVLA (Ours)}
& \textbf{82}
& \textbf{78}
& \textbf{72}
& \textbf{56}
& \textbf{66}
& \textbf{62} \\
\thickhline
\end{tabular}
}
\vspace{-8pt}
\end{table*}

==> tabs/temporal_comp.tex <==
\begin{table*}[t]
\centering
\caption{
\small\textbf{Quantitative comparison results with temporal-context VLA models across three simulation benchmarks~\cite{liu2023libero,li2025evaluating,cherepanov2026memory} (\S\ref{supp:temporal_baselines}).}
Success rates (\%) are reported.
The LIBERO average is computed over the first four suites because most VLA models do not report results on Long-90.
}
\label{tab:temporal_baselines}

% ================= SimplerEnv-Bridge =================
{\small\textbf{(a) SimplerEnv-Bridge}}
\vspace{2pt}

\resizebox{0.9\linewidth}{!}{
\setlength\tabcolsep{14pt}
\renewcommand\arraystretch{1.0}
\begin{tabular}{l|c|ccccc}
\thickhline
\rowcolor{mygray}
Method
& Publication
& \makecell{Spoon\\on Towel}
& \makecell{Carrot\\on Plate}
& \makecell{Stack\\Cube}
& \makecell{Eggplant\\in Basket}
& \makecell{Avg.\\Success} \\
\hline
\hline
TraceVLA~\citep{zheng2025tracevla}
& ICLR2025
& 12.5 & 16.6 & 16.6 & 65.0 & 27.7 \\

RoboVLMs~\citep{li2024towards}
& ArXiv2024
& 45.8 & 20.8 & 4.2 & 79.2 & 37.5 \\

CronusVLA~\citep{li2026towards}
& AAAI2026
& 66.7 & 54.2 & 20.8 & \textbf{100.0} & 60.4 \\

MemoryVLA~\citep{shi2025memoryvla}
& ICLR2026
& 75.0 & \textbf{75.0} & 37.5 & \textbf{100.0} & 71.9 \\
\hline
\ourmethod~\textbf{(Ours)}
& --
& \textbf{83.3} & \textbf{75.0} & \textbf{41.7}
& 95.8 & \textbf{73.9} \\
\hline
\end{tabular}
}

\vspace{7pt}

% ================= LIBERO =================
{\small\textbf{(b) LIBERO}}
\vspace{2pt}

\resizebox{0.9\linewidth}{!}{
\setlength\tabcolsep{14pt}
\renewcommand\arraystretch{1.0}
\begin{tabular}{l|c|ccccc}
\thickhline
\rowcolor{mygray}
Method
& Publication
& Spatial
& Object
& Goal
& Long-10
& \makecell{Avg.\\Success} \\
\hline
\hline
TTF-VLA~\citep{liu2026ttf}
& AAAI2026
& 84.0 & 73.0 & 81.0 & 58.0 & 74.0 \\

TraceVLA~\citep{zheng2025tracevla}
& ICLR2025
& 84.6 & 85.2 & 75.1 & 54.1 & 74.8 \\

4D-VLA~\citep{zhang20264d}
& NeurIPS2025
& 88.9 & 95.2 & 90.9 & 79.1 & 88.6 \\

MemoryVLA~\citep{shi2025memoryvla}
& ICLR2026
& 98.4 & 98.4 & 96.4 & 93.4 & 96.7 \\

CronusVLA~\citep{li2026towards}
& AAAI2026
& 97.3 & \textbf{99.6} & 96.9 & 94.0 & 97.0 \\
\hline
\ourmethod~\textbf{(Ours)}
& --
& \textbf{98.8} & 99.0 & \textbf{97.2}
& \textbf{95.8} & \textbf{97.7} \\
\hline
\end{tabular}
}

\vspace{7pt}

% ================= MIKASA-Robo =================
{\small\textbf{(c) MIKASA-Robo}}
\vspace{2pt}

\resizebox{0.9\linewidth}{!}{
\setlength\tabcolsep{14pt}
\renewcommand\arraystretch{1.0}
\begin{tabular}{l|c|cccccc}
\thickhline
\rowcolor{mygray}
Method
& Publication
& \makecell{ShellGame\\Touch}
& \makecell{Intercept\\Medium}
& \makecell{Remb.\\Color-3}
& \makecell{Remb.\\Color-5}
& \makecell{Remb.\\Color-9}
& \makecell{Avg.\\Success} \\
\hline
\hline
CronusVLA~\citep{li2026towards}
& AAAI2026
& 32 & 5 & 31 & 13 & 9 & 18.0 \\

MemoryVLA~\citep{shi2025memoryvla}
& ICLR2026
& 88 & 24 & 44 & 30 & 20 & 41.2 \\
\hline
\ourmethod~\textbf{(Ours)}
& --
& \textbf{94} & \textbf{43} & \textbf{58}
& \textbf{37} & \textbf{25} & \textbf{51.4} \\
\hline
\end{tabular}
}
\end{table*}
